Multi-Track Timeline Control for Text-Driven 3D Human Motion Generation

Recent advances in generative modeling have led to promising progress on synthesizing 3D human motion from text, with methods that can generate character animations from short prompts and specified durations. However, using a single text prompt as input lacks the fine-grained control needed by animators, such as composing multiple actions and defining precise durations for parts of the motion. To address this, we introduce the new problem of timeline control for text-driven motion synthesis, which provides an intuitive, yet fine-grained, input interface for users. Instead of a single prompt, users can specify a multi-track timeline of multiple prompts organized in temporal intervals that may overlap. This enables specifying the exact timings of each action and composing multiple actions in sequence or at overlapping intervals. To generate composite animations from a multi-track timeline, we propose a new test-time denoising method. This method can be integrated with any pre-trained motion diffusion model to synthesize realistic motions that accurately reflect the timeline. At every step of denoising, our method processes each timeline interval (text prompt) individually, subsequently aggregating the predictions with consideration for the specific body parts engaged in each action. Experimental comparisons and ablations validate that our method produces realistic motions that respect the semantics and timing of given text prompts. Our code and models are publicly available at https://mathis.petrovich.fr/stmc.

==> 6_acknowledgements_short.tex <==
\medskip 

{ \small %
\noindent\textbf{Acknowledgements.}
This work was granted access to
the HPC resources of IDRIS under the allocation 2023-AD011012129R3 made by GENCI.
GV acknowledges the ANR project CorVis ANR-21-CE23-0003-01.
The authors would like to thank Nicolas Dufour for the interesting discussions on diffusion models.

\noindent\textbf{MJB Disclosure}: \url{https://files.is.tue.mpg.de/black/CoI_CVPR_2024.txt}
\par
}






==> mymath.tex <==
\newcommand{\defeq}{\stackrel{\tiny\mathrm{def}}{=}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\thalf}{\tfrac{1}{2}}


\newcommand{\E}{\operatorname{\mathsf E}}
\newcommand{\K}{\operatorname{\mathsf K}}
\newcommand{\Var}{\operatorname{\mathsf Var}}
\renewcommand{\H}{\operatorname{\mathsf H}}
\newcommand{\I}{\operatorname{\mathsf I}}
\newcommand{\D}{\operatorname{\mathsf D}}
\newcommand{\Cov}{\operatorname{\mathsf Cov}}
\newcommand{\FIM}{\operatorname{\mathcal{F}}}


\newcommand{\R}{\operatorname{\mathbb R}}
\newcommand{\Z}{\operatorname{\mathbb Z}}
\newcommand{\X}{\operatorname{\mathcal X}}
\newcommand{\Y}{\operatorname{\mathcal Y}}


\newcommand{\MVN}{\operatorname{MVN}}
\newcommand{\Normal}{\operatorname{Normal}}
\newcommand{\Beta}{\operatorname{Beta}}
\newcommand{\Bernoulli}{\operatorname{Bernoulli}}
\newcommand{\Categorical}{\operatorname{Categorical}}
\newcommand{\Shuffle}{\operatorname{Shuffle}}


\newcommand{\sign}{\operatorname{sign}}
\newcommand{\logit}{\operatorname{logit}}
\newcommand{\expit}{\operatorname{expit}}
\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\softplus}{\operatorname{softplus}}
\newcommand{\logsumexp}{\operatorname{logsumexp}}
\DeclareMathOperator*{\argmin}{\operatorname{\arg\min}}
\DeclareMathOperator*{\argmax}{\operatorname{\arg\max}}
\DeclareMathOperator*{\arginf}{\operatorname{\arg\inf}}
\DeclareMathOperator*{\argsup}{\operatorname{\arg\sup}}


\newcommand{\tee}{\mathsf{\tiny T}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\zeros}{\operatorname{\mathbb{0}}}
\newcommand{\ones}{\operatorname{\mathbb{1}}}
\newcommand{\eye}{\operatorname{I}}


\newcommand{\Encoder}{\operatorname{Encoder}}
\newcommand{\Decoder}{\operatorname{Decoder}}
\newcommand{\MLP}{\operatorname{MLP}}
\newcommand{\ResNet}{\operatorname{ResNet}}
\newcommand{\Augment}{\operatorname{Augment}}


\renewcommand{\dot}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ceil}[1]{\left\lceil #1 \rceil|}
\newcommand{\floor}[1]{\left\lfloor #1 \rfloor|}
\DeclareMathOperator*{\bigtimes}{\times}


\newcommand{\domain}{\operatorname{domain}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\ndims}{\operatorname{ndims}}
\newcommand{\shape}{\operatorname{shape}}
\newcommand{\size}{\operatorname{size}}
\newcommand{\len}{\operatorname{len}}
\newcommand{\indexes}{\operatorname{indexes}}



\theoremstyle{plain}            %
\newtheorem{thm}{Theorem}[section]
\newtheorem{lma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{clm}[thm]{Claim}

\theoremstyle{definition}       %
\newtheorem{defn}[thm]{Definition}
\newtheorem{examp}[thm]{Example}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{rmk}[thm]{Remark}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}

==> mypackages.tex <==
\usepackage[utf8]{inputenc}

\usepackage[T1]{fontenc}


\usepackage[numbers]{natbib} %

\usepackage{verbatim}
\usepackage[sumlimits,]{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{srcltx}

\usepackage{tocloft}
\renewcommand\cftsecleader{\cftdotfill{\cftdotsep}}
\usepackage{bm}

\usepackage[bb=boondox]{mathalfa}   %


\usepackage{array}
\usepackage{graphics,graphicx,psfrag,epsfig}
\usepackage{wrapfig}
\graphicspath{{.} {./figures/}}

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

\usepackage[parfill]{parskip}
\usepackage{geometry}

\usepackage{xcolor}
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
\definecolor{deeporange}{rgb}{0.6,0.25,0}
\definecolor{verylightgray}{rgb}{0.97,0.97,0.97}
\definecolor{bluegray}{rgb}{0.3,0.3,0.6}

\usepackage[
    colorlinks=true,
    linkcolor=black,       urlcolor=bluegray,
    anchorcolor=bluegray,  filecolor=bluegray,
    menucolor=bluegray,    citecolor=bluegray
]{hyperref}


\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{cleveref}
\usepackage{cancel}
\usepackage{ulem}
\newcommand{\stkout}[1]{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}



\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{8} %
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{8}  %

\usepackage{listings}
\usepackage{textcomp}  %




\lstdefinestyle{pythonstyle}{
  language=Python,
  basicstyle=\footnotesize\ttm,
  keywordstyle=\ttb\color{deepblue},
  commentstyle=\ttm\color{deepgreen},
  stringstyle=\color{deeporange},
  emphstyle=\ttb\color{deepred},
  backgroundcolor=\color{verylightgray},
  emph={__init__, __call__},      %
  morekeywords = {self,yield},
  showspaces=false,               %
  showstringspaces=false,         %
  showtabs=false,                 %
  frame=single,                   %
  tabsize=2,                      %
  captionpos=b,                   %
  breaklines=false,               %
  breakatwhitespace=false,        %
  columns=fullflexible,           %
  extendedchars=false,
  keepspaces=true,
  upquote=true,                   %
  literate={-}{-}1 {*}{*}1
}


\lstnewenvironment{python}[1][]
{
\lstset{style=pythonstyle}
\lstset{#1}
}
{}

\newcommand\pythoninline[1]{{\lstset{style=pythonstyle}\lstinline!#1!}}
\renewcommand{\v}[1]{\pythoninline{#1}}

\newcommand\pythoninput[1]{\lstinputlisting[style=pythonstyle]{#1}}
